Interferometry of chemically peculiar stars: theoretical predictions vs. modern observing facilities

By means of numerical experiments we explore the application of interferometry to the detection and characterization of abundance spots in chemically peculiar (CP) stars using the brightest star eps~Uma as a case study. We find that the best spectral regions to search for spots and stellar rotation signatures are in the visual domain. The spots can clearly be detected already at a first visibility lobe and their signatures can be uniquely disentangled from that of rotation. The spots and rotation signatures can also be detected in NIR at low spectral resolution but baselines longer than 180~m are needed for all potential CP candidates. According to our simulations, an instrument like VEGA (or its successor e.g., FRIEND) should be able to detect, in the visual, the effect of spots and spots+rotation, provided that the instrument is able to measure $V^2\approx10^{-3}$, and/or closure phase. In infrared, an instrument like AMBER but with longer baselines than the ones available so far would be able to measure rotation and spots. Our study provides necessary details about strategies of spot detection and the requirements for modern and planned interferometric facilities essential for CP star research.

==> tables/stars-short.tex <==
\begin{center}
\begin{table*}
\caption{Observability of CP stars with modern and future interferometers. The full table is available online.}
\label{tab:stars}
\begin{tabular}{ccccccccccccc}
\hline
HD      & $V$  &  $J$  & $H$  & $K$  &  $d$  & $R$     & $\theta$  & \multicolumn{4}{c}{$B_{\rm max}^{\dagger}$}             & ref. \\ %&  Instrument\\
number & mag  &  mag  & mag  & mag  &  pc   & $\Rsun$ & mas       & \multicolumn{4}{c}{m}                                   & \\ %& \\
       &      &       &      &      &       &         &           & $0.55$~\mum  & $1.25$~\mum & $1.65$~\mum  & $2.15$~\mum & \\ %& \\
\hline                                       
\multicolumn{13}{c}{Magnetic CP stars}\\
\hline
24712    & 6.00  & 5.43  & 5.31  & 5.26  &  49.2  & 1.46  & 0.28  &   296 &   674 &   890 &  1160 & 1  \\ %& 5, 9, 10f, 11\\
37776    & 6.96  & 7.29  & 7.42  & 7.42  & 330.0  & 2.75  & 0.08  &  1215 &  2762 &  3646 &  4751 & 2  \\ %&\\
40312    & 2.62  & 2.69  & 2.70  & 2.75  &  50.8  & 4.58  & 0.84  &   148 &   336 &   444 &   578 & 1  \\ %& 5, 9, 10, 11\\
65339    & 6.02  &  ...  &  ...  &  ...  &  98.7  & 4.55  & 0.43  &   509 &  1157 &  1527 &  1990 & 1  \\ %& 10f\\
101065   & 8.03  & 7.11  & 6.94  & 6.92  & 112.0  & 1.98  & 0.16  &   689 &  1567 &  2069 &  2696 & 1  \\ %&\\
128898   & 3.19  & 2.84  & 2.73  & 2.74  &  16.6  & 1.94  & 1.09  &   104 &   236 &   312 &   407 & 1  \\ %& 5, 6, 7, 9, 10, 11\\
137909   & 3.68  & 3.38  & 3.28  & 3.28  &  34.3  & 2.47  & 0.67  &   169 &   384 &   507 &   661 & 1  \\ %& 5, 9, 10f, 11\\
137949   & 6.69  & 6.31  & 6.28  & 6.25  &  88.7  & 2.13  & 0.22  &   507 &  1153 &  1522 &  1984 & 1  \\ %& 10f\\
201601   & 4.68  & 4.28  & 4.18  & 4.10  &  36.3  & 2.07  & 0.53  &   213 &   486 &   641 &   835 & 1  \\ %& 5, 9, 10f, 11\\
\multicolumn{13}{c}{\dots}\\
\hline
\multicolumn{13}{c}{HgMn stars}\\ %
\hline
358      & 2.06  & 2.30  & 2.33  & 2.37  &  29.7  & 2.48  & 0.78  &   142 &   323 &   427 &   556 & 6  \\ %& 5, 9, 10, 11\\
11753    & 5.11  & 5.17  & 5.25  & 5.17  &  94.1  & 9.50  & 0.94  &   407 &   926 &  1222 &  1593 & 7  \\ %& 10f, 11\\
32964    & 5.12  & 5.23  & 5.22  & 5.20  &  94.7  & 2.40  & 0.24  &   597 &  1358 &  1793 &  2336 & 8  \\ %& 10f\\
33904    & 3.29  & 3.53  & 3.59  & 3.57  &  57.0  & 3.39  & 0.55  &   205 &   466 &   615 &   801 & 9  \\ %& 5, 9, 10f, 11\\
34364    & 6.14  & 6.19  & 6.25  & 6.26  & 122.1  & 3.70  & 0.28  &   788 &  1792 &  2366 &  3083 & 10 \\ %&\\
\hline
\end{tabular}
\begin{flushleft}
\medskip
$^{\dagger}$~--~{maximum baseline length needed to fully resolve the star at a given wavelength.}
\par\medskip
\textbf{References:}
(1)~\citet{2006A&A...450..763K}; (2)~\citet{2000AstL...26..177K}; (3)~\citet{2008CoSka..38..245F};
(4)~\citet{2011MNRAS.417..444P}; (5)~\citet{2011MNRAS.417..444P}; (6)~\citet{2002ApJ...575..449A};
(7)~\citet{2012A&A...539A.142M}; (8)~\citet{2011A&A...529A.160M}; (9)~\citet{2011A&A...534L..13K};
(10)~\citet{2010MNRAS.407.2383F}
\end{flushleft}
\end{table*}
\end{center}

